Optimally Guarding Perimeters and Regions with Mobile Range Sensors

We investigate the problem of using mobile robots equipped with 2D range sensors to optimally guard perimeters or regions, i.e., 1D or 2D sets. Given such a set of arbitrary shape to be guarded, and $k$ mobile sensors where the $i$-th sensor can guard a circular region with a variable radius $r_i$, we seek the optimal strategy to deploy the $k$ sensors to fully cover the set such that $\max r_i$ is minimized. On the side of computational complexity, we show that computing a $1.152$-optimal solution for guarding a perimeter or a region is NP-hard, i.e., the problem is hard to approximate. The hardness result on perimeter guarding holds when each sensor may guard at most two disjoint perimeter segments. On the side of computational methods, for the guarding perimeters, we develop a fully polynomial time approximation scheme (FPTAS) for the special setting where each sensor may only guard a single continuous perimeter segment, suggesting that the aforementioned hard-to-approximate result on the two-disjoint-segment sensing model is tight. For the general problem, we first describe a polynomial-time (2+$\epsilon)$-approximation algorithm as an upper bound, applicable to both perimeter guarding and region guarding. This is followed by a high-performance integer linear programming (ILP) based method that computes near-optimal solutions. Thorough computational benchmarks as well as evaluation on potential application scenarios demonstrate the effectiveness of these algorithmic solutions.

==> texs/03-complexity-backup.tex <==
In this section, we prove the problem of finding the minimum radius 
for guarding the perimeter or the interior of a region with range 
sensors is strongly NP-hard to approximate within $\alpha = 2\sqrt{3}/3 
\approx 
1.155$. That is, we show that \osgt is computationally hard to 
approximate. Furthermore, the inapproximability gap remains 
for \opgt even when each robot can only guard two disconnected 
boundary segments.

For the main result on \osgt inapproximability is proven in two 
steps. First in Section~\ref{complexity:3netcomp}, starting from 
a planar graph with maximum degree $3$, we construct a structure 
which we call {\em $3$-net} and prove that finding the minimum 
coverage radius of the $3$-net is NP-hard to approximate within 
$\alpha$. 
%
Then, in Section~\ref{subsec:osgthard}, we apply a straightforward 
reduction to transform the $3$-net to a simple polygon (i.e., 
polygon without self-intersections or holes), followed by a 
second reduction to convert the $3$-net to a simple polygon and 
prove the hardness of boundary guarding when each robot can only 
guards two disjoint continuous boundary segments.
%
In Section~\ref{subsec:2-seghard}, we show the inapproximability
of the special \opgt setup. 

\begin{comment}
Our proof uses vertex cover \cite{garey1977rectilinear} for 
the reduction, which is NP-complete on planar graphs with a maximum 
degree of $3$. We will use planar graphs that are $3$-regular (this 
is not necessary but makes the proof much shorter overall). For 
completeness, we provide a lemma bridging the results. 

\begin{lemma}
Vertex cover on planar 3-regular graphs is NP-complete.
\end{lemma}
\begin{proof}
Given a planar graph $G$ with max degree $3$, for each vertex $v$ of 
degree two or less, attach the structure shown in 
Fig.~\ref{fig:structural_aug} to $u$ until it reaches degree $3$. 
It is clear that the conversion preserves the hardness of vertex 
cover.
\begin{figure}[!ht]
\vspace*{-3mm}
    \centering
		\begin{small}
    \begin{overpic}[scale=0.3]{../figures/structure_augment}
        \put(38,30){\color{black}$u$}
        \put(56,30){\color{black}$w$}
    \end{overpic}
		\end{small}
\vspace*{-3mm}
    \caption{A structural gadget attached to a vertex $u$. With the 
		augmentation, the degree of $u$ will increase by $1$ while the 
		size of minimum vertex cover will increase by $3$, regardless of 
		whether $u$ is part of a vertex cover or not.}
    \label{fig:structural_aug}
\end{figure}
\end{proof}
%With at most two such structural augmentations per vertex, a planar 
%graph with maximum degree $3$ can be turned into a planar $3$-regular 
%graph. It is s\traightforward to see that the reduction preserves 
\end{comment}

\subsection{Hardness on Optimally Guarding a $3$-Net}\label{complexity:3netcomp}
\subsubsection{Constructing $3$-nets}
Starting from a planar graph $G$ with maximum degree $3$, we construct 
a structure that we call the $3$-net (following \cite{feder1988optimal}). 
First, an edge $uw \in E(G)$ is converted to a path $uv_1, v_1v_2, 
\ldots, v_{2m}w$ where $m\ge 2$ is an integer to be decided later. We 
denote such a path as $u\cdots w$; each edge along $u\cdots w$ is straight 
and has unit edge length. We also require that each path is nearly straight 
locally. We will make this point more precise later.
%
For a vertex of $G$ with degree $3$, e.g., a vertex $u \in V(G)$ 
neighboring $w, x, y \in V(G)$, we choose proper lengths for 
paths, $u\cdots w$, $u\cdots x$, and $u\cdots y$ such that
these paths meet at $u$ forming pairwise angles of $2\pi/3$. Clearly, 
the same can be ensured for vertices of $G$ of degree $2$, which 
is applied. At the global scale, we also require that any two 
paths converted from edges of $G$ are at least distance $2$ away 
from each other except when they share a common end vertex. 
The construction so far converts $G$ to a new graph $G'$, which 
forms the backbone of the $3$-net. Fig.~\ref{fig:backbone} sketches 
such a $G'$ (right) constructed from a $5$ vertex graph with 
maximum vertex degree $3$ (right).
\begin{figure}[!ht]
    \centering
		\begin{small}
    \begin{overpic}[width=0.8\columnwidth]{../figures/backbone.png}
    \end{overpic}
		\end{small}
    \caption{Siwei: draw some dots on the paths, but not bars.}
    \label{fig:backbone}
\end{figure}
\end{proof}

From the backbone, a second modification is made which completes the 
construction. For each path $u\cdots w = uv_1\ldots v_{2m}w$ in $G'$ 
that is previously constructed, for each $v_iv_{i+1}$, $1 \le i
\le 2m-1$, we add a line segment of length $\sqrt{3}$ that is 
perpendicular to $v_iv_{i+1}$ such that $v_iv_{i+1}$ and the line 
segment divide each other in the middle. A graphical illustration is
given in Fig.~\ref{fig:path-bar}. We note that the bars do not need 
to be connected to the backbone $G'$. $G'$ and the bars form the 
$3$-net, which we denote as $T_G$. An illustration of $T_G$ constructed
from the backbone in Fig.~\ref{fig:backbone} is given in 
Fig.~\ref{fig:3-net}.
\begin{figure}[!ht]
\vspace*{-4mm}
    \centering
    \includegraphics[scale=0.3]{../figures/edgepath.eps}
\vspace*{-4mm}
    \caption{Structure within the odd length path and attached 
		perpendicular ``bars'' with length $\sqrt{3}$. Regarding the 
		representation of such non-integral coordinates in the problem 
		input, a precise enough fractional representation is enough 
		for the proof due to the inapproximability gap in the result.}
    \label{fig:path-bar}
\end{figure}

\begin{figure}[!ht]
\vspace*{-2mm}
    \centering
    \begin{overpic}[scale=0.4]{../figures/structure.eps}
    \put(53,36){\color{black}$w$}
		\end{overpic}
\vspace*{-1mm}
    \caption{Part of a $3$-net $T$ constructed from a $3$-regular 
		graph.}
    \label{fig:3-net}
\end{figure}


As an intermediate step, we work with a $3$-net structure 
\cite{feder1988optimal} constructed as follows. Starting from a planar 
$3$-regular graph $G$, we replace each edge with a (possibly curved) 
path of odd length large than 3. The goal is to obtain a new graph 
in which a vertex where the replaced edges used to meet now have three 
edges forming an angle of $2\pi/3$ pairwise at the vertex. 
%
As an illustration, the structure in Fig~\ref{fig:structural_aug} converts
to a structure shown in Fig.~\ref{fig:3-net} where the new edges at $w$ 
all meet at angle of $2\pi/3$. The edge $uw$ in 
Fig.~\ref{fig:structural_aug} becomes a edge of some odd length $2m + 1$. 
%
Subsequently, these odd length edges are subdivided into unit length 
edges. The edge $uw$ from Fig.~\ref{fig:structural_aug} then becomes 
$2m + 1$ edges $uv_1, v_1v_2, \ldots, v_{2m}w$ in a new graph $G'$ 
(part of which is shown in Fig.~\ref{fig:3-net}). We denote the path 
between $uw$ as $u\cdots w$. $m$ is chosen to be sufficiently large 
such that the local curvature along $u\cdots w$ is sufficiently small,
as will bee needed later constructions. 
% Denote $L$ as the total path length. 

Then, for each unit length edge on the path $u\cdots w$, e.g., $v_iv_{i+1}$, 
we add a straight line of length $\sqrt{3}$ that crosses $v_iv_{i+1}$ 
in the middle and form a right angle with $v_iv_{i+1}$. There form the 
vertical bars in Fig.~\ref{fig:path} which on a larger scale are the 
spikes on $G'$ (see Fig.~\ref{fig:3-net}). We note that these bars are
not part of $G'$. The overall structure ($G'$ and the bars) form the 
$3$-net $T$. Let $L$ be the number of (unit length) edges of $G'$ (i.e., 
$L = \sum_{uv \in E(G)}len(u\cdots w)$). 

Having shown the basic construction of a $3$-net $T$, we are ready to 
prove the following.

\begin{theorem}\label{t:3nethard}
Covering of a $3$-net using $(\frac{L-|E|}{2}+k)$ circular discs while 
minimizing the maximum disc radius is NP-hard to approximate within a 
factor of $\alpha = 2\sqrt{3}/3$.
\end{theorem}
\begin{proof}
Following the reasoning of \cite{feder1988optimal}, which is not repeated
here, the $3$-net $T$ may be obtained in polynomial time from a 
$3$-regular graph. We now take a closer look at the odd length path between 
two neighboring pair of vertices on $T$.

For a path $u\cdots w$ on $T$, 
consider the endpoints of the associated vertical bars. To cover 
four such endpoints, a circle needs a radius of at least $1$. For the 
partial $3$-net structure from Fig.~\ref{fig:path}, the optimal covering 
strategy must always be one of the two cases illustrated in 
Fig.~\ref{fig:pathcover}.  The next possible covering of four end 
points is when a circle reaches a radius of $\alpha=2\sqrt{3}/3 \approx 
1.155$, where a circle can cover three endpoints from one side of 
$u\cdots w$ and one endpoint from the other side of $u \cdots w$. 
(see Fig.~\ref{fig:pathcovert}).
\begin{figure}[!ht]
\vspace*{-3mm}
    \centering
    \includegraphics[scale=0.3]{../figures/edgepath1.eps}\vspace{3mm}
    \includegraphics[scale=0.3]{../figures/edgepath2.eps}
\vspace*{-5mm}
   \caption{Two coverage patterns on an odd length path with robots of 
		range sensing radius $1$ which is less than $\alpha$.}
    \label{fig:pathcover}
\end{figure}

\begin{figure}[!ht]
    \centering
    \includegraphics[scale=0.33]{../figures/edgepath3.eps}
    \caption{Asymmetrical coverage of four endpoints using a circle of 
		radius $\alpha = 2\sqrt{3}/3$.}
    \label{fig:pathcovert}
\end{figure}

If the planar $3$-regular graph has a vertex cover of size $k$, 
then place $k$ robots at the corresponding vertex on $T$ (which 
covers a junction where three edges meet at angles of $2\pi/3$) 
and let the rest cover the rest of the paths and bars in patterns 
as illustrated in Fig.~\ref{fig:pathcover} then the $3$-net $T$ can 
be guarded with $(\frac{L-|E|}{2}+k)$ robots with maximum sensing 
radius radius $1$.

On the other hand, if the $3$-net $T$ can be covered with 
$(\frac{L-|E|}{2} +k)$ circles with radii less than $\alpha$, for 
each odd length path $u\cdots w$, it takes at least 
$(len(u\cdots w)-1)/2$ circles to cover all the bars on it while 
touching at most one of $u$ and $w$. Therefore, the vertices 
corresponding to the rest $k$ centers of the circle yields a vertex 
cover of size $k$ of the previous planar 3 regular graph. 
\end{proof}
% \sw{It can probably be improved to 19/16 = 1.19 or even sqrt(7)/2 = 1.32.}

% Replace each edge with an path with length larger than 3 and is an odd number to get $G'$, let $L$ be the total length. 

% 1. If the $G$ has a vertex cover of size k. Then $G'$ can be covered with $k+(L-|E|)/2$ disks.

% 2. If $G'$ can be covered with $k+(L-|E|)/2$ disks.

\subsection{From $3$-Nets to Simple Polygons}\label{subsec:osgthard}
We now proceed to show that \osgt is hard to approximate by converting
a $3$-net into a simply polygon. Along the backbone $G'$ of a $3$-net 
$T$, we first expand the lines segments by $\delta$ to get a 2D region  
(see Fig.~\ref{fig:door}(a)). We may describe the interior of the resulting 
polygon as 
\[P=\{p\in \R^2\ |\ \min_{q\in T}(\|p-q\|_1)\leq \delta/2\}\]

For small enough $\delta$, it's clear that $P$ is a polygon with holes.
Let $K = (\frac{L-|E|}{2}+k)$, it holds that
\begin{align*}
&size(K, T) \leq               size(K, P)\leq size(K, T) + \delta,\\
&size(K, T) \leq      size(K, \partial P)\leq size(K, T) + \delta.
\end{align*}
To convert the structure into a simple polygon, we can open ``doors'' of 
width $\delta$ on the structure to get rid of the holes (see 
Fig.~\ref{fig:door}(b)). Each opening removes one hole from $P$. This is 
straightforward to check; we omit the details. 
\begin{figure}[ht]
		\centering
		\vspace*{-2.5mm}
    \begin{small}
    \includegraphics[scale=.3]{../figures/holes.eps} 
    \begin{overpic}[scale=.3]{../figures/doors.eps}
        \put(53,42){$\delta$}
        \put(-55,5){(a)}
        \put(53,5){(b)}
    \end{overpic}
	  \end{small}
		\vspace*{-3mm}
    \caption{(a) A $3$-net $T$ maybe readily converted into a simple polygon 
		$P$ with holes by expanding along its backbone. (b) Creating a ``door'' 
		of width $\delta$ will remove one hole from $P$.}
    \label{fig:door}
\end{figure}

Denoting the resulting simple polygon as $P'$, we have
\begin{align*}
&size(K, P) - \delta  \leq               size(K, P')\leq size(K, P),\\
&size(K, \partial P) - \delta  \leq      size(K, \partial P')\leq size(K, \partial P).
\end{align*}

Therefore, both $size(k, P')$ and $size(k, \partial P')$ are between 
$size(k, T) - \delta$ and $size(k, T) + \delta$. Suppose the \osgt for 
$\partial P'$ or $P'$ has a polynomial approximation algorithm with 
approx ratio $1.155 - \epsilon$ where $\epsilon > 0$, let $\delta = 
\epsilon/2$, then the optimal guarding problem for the $3$-net $T$ can 
be approximated within 1.155. However, by Theorem~\ref{t:3nethard}, 
it is hard to find the optimal coverage radius of $T$. This proves 
the following

\begin{theorem}\label{t:osgthard}
\osgt is NP-hard and does not admit a polynomial time approximation 
within a factor of $(1 + \alpha)$ with $\alpha = 2\sqrt{3}/2$, unless 
P$=$NP.
\end{theorem}

\subsection{\opgt with Sensor Guarding Segment Restrictions}\label{subsec:2-seghard}
The inapproximability gap from Theorem~\ref{t:osgthard} prompts us to 
further consider restriction on the setup with the hope that meaningful 
yet more tractable problems may arise. On natural restriction is to 
limit the number of continuous segments a mobile sensor may cover. As 
will be shown in Section~\ref{subsec:singleseg}, if a mobile sensor may 
only guard a single continuous perimeter segment, a 
$(1 + \varepsilon)$-optimal solution can be computed efficiently. 
On the other hand, it turns out that if a sensor can guard up to two 
continuous perimeter segments, \opgt remains hard to approximate. 

%that a single robot may only cover some fixed number of continuous boundary segments $c$. In the construction in ~\ref{complexity:simp}, each robot with coverage radius less than $\alpha$ can cover no more than $3$ disconnected boundary segments. Meaning the restriction of $c=3$ will still keep most of the hardness properties.

%Further, in the case of posing an even stricter limitation that each robot can only cover no more than two $2$ disconnected boundary segments, one may hope to get even a PTAS, since it is somewhat reminiscent of the edge-cover problem which admits efficient polynomial algorithm\cite{garey1979computers}. Unfortunately, like the unrestricted version of problem, it's still NP-hard to approximate within $\alpha$.

As we have mentioned, the use of $3$-regular graph in constructing the 
$3$-net structure is not a must, but a convenience. 

With a careful analysis on the vertices on the ``3-net'', it can be confirmed the reduction does not rely on the 3-regular property of the initial graph, and works for vertex with degree of $1$ or $2$ as well (the reduction in previous section used the 3-regular just for the simplicity of explanation). With this, we made some modifications illustrated in Fig.~\ref{fig:even3net} on the structure of the planar graph with maximum degree 3 constructed in \cite{garey1977rectilinear}. For an edge connecting different vertex cycles, we create another parallel edge adhere to it, do the same thing for the edge between inner vertex and outer vertex cycle.
Under this setting, the hardness property still remains while each vertex has an even degree, either $2$ or $4$.

\begin{figure}[!ht]
    \centering
    \includegraphics[scale=0.30]{../figures/before.eps}
    \includegraphics[scale=0.30]{../figures/after.eps}
    \caption{``3-net'' with even degree. The left picture is the original structure replacement in \cite{garey1977rectilinear}. In short, for a vertex $u$ with degree $n$ in a planar graph, convert it into a cycle structure with $2n + 1$ vertices, $a_u(1), b_u(1), \dots, a_u(n), b_n(n)$ is the outer vertex cycle, $z_u$ is connected to $b_u(n)$ and $a_u(i)$ $1\leq i \leq n$ is connected to other $a_v(i')$ for each edge $uv$. In this case, whether that vertex is taken in the vertex cover of the original graph corresponds to $n$ or $n+1$ vertices taken from the vertex cycle and inner vertex in the vertex cover of the transformed graph. Additionally, we add a parallel edge to $z_u b_u(n)$ and each $a_u(i)$ and $a_v(i')$, such that each vertex's degree is even. Note that the paths transformed from each pair of paralleled edge can be viewed as ``adhere'' to each other which we will explain later.}
    \label{fig:even3net}
\end{figure}

With each vertex's degree even, there exists a Eulerian tour along
the paths with non-paralleled and paralleled paths as Fig.~\ref{fig:path_exp}. Image drawing along the Eulerian tour will create the skeleton of the polygon.

% To eliminate some possible self intersections like Fig.~\ref{fig:intersection}, 

\begin{figure}[!ht]
    \centering
    \includegraphics[scale=0.28]{../figures/1going.eps}
    \includegraphics[scale=0.28]{../figures/2going.eps}
    \caption{The left and right picture corresponds to whether or not the path has a parallel path of it respectively.}
    \label{fig:path_exp}
\end{figure}
\begin{figure}[!ht]
    \centering
    \begin{subfigure}[!htb]{0.26\textwidth}
        \centering
        \includegraphics[width=\textwidth]{../figures/t3}
        \caption{Intersection}
        \label{fig:intersection}
    \end{subfigure}
    \hfill
    \begin{subfigure}[!htb]{0.18\textwidth}
        \centering
        \includegraphics[width=\textwidth]{../figures/t4}
        \includegraphics[width=\textwidth]{../figures/t5}
        \caption{Two solutions}
        \label{fig:solution}
    \end{subfigure}
        \caption{In order to eliminate some possible self-intersections as ~\ref{fig:intersection}, transform it into one of the solutions in ~\ref{fig:solution} to make the Eulerian tour remain connected (it is clear that one of the two solutions will satisfy this).}
        \label{fig:eliminter}
\end{figure}

After some adjustments to such self-intersections, a Non self-intersected tour along the ``3-net'' can be obtained. One side of the tour will be an unbounded area while the other side is a simple polygon. So, such tour can be the boundary of a simple polygon.

While near the junction of the original $D_N$, the boundary will be either one of the below that the solution to the optimal guarding of the boundary will only cover two disconnect boundary segments.

\begin{figure}[!ht]
    \centering
    \includegraphics[scale=.29]{../figures/t1}
    \includegraphics[scale=.29]{../figures/t2}
    \caption{The figure shows two possible types of boundary near the vertex with degree of $4$ before the transformation. Therefore, a robot near the vertex will only be able to cover two disconnected boundary segments with sensing radius less than $\alpha$ if the solution is optimal.}
    \label{fig:2types}
\end{figure}

With this, we conclude that,
\begin{theorem}\label{them:twoconthard}
Optimal guarding problem for boundary of a simple polygon cannot be approximated within $\alpha$ even when the edge length is bounded, and each robot can guard no more than two boundary segments unless P=NP.
\end{theorem}
